High precision determination of the gluon fusion Higgs boson cross-section at the LHC

We present the most precise value for the Higgs boson cross-section in the gluon-fusion production mode at the LHC. Our result is based on a perturbative expansion through N$^3$LO in QCD, in an effective theory where the top-quark is assumed to be infinitely heavy, while all other Standard Model quarks are massless. We combine this result with QCD corrections to the cross-section where all finite quark-mass effects are included exactly through NLO. In addition, electroweak corrections and the first corrections in the inverse mass of the top-quark are incorporated at three loops. We also investigate the effects of threshold resummation, both in the traditional QCD framework and following a SCET approach, which resums a class of $\pi^2$ contributions to all orders. We assess the uncertainty of the cross-section from missing higher-order corrections due to both perturbative QCD effects beyond N$^3$LO and unknown mixed QCD-electroweak effects. In addition, we determine the sensitivity of the cross-section to the choice of parton distribution function (PDF) sets and to the parametric uncertainty in the strong coupling constant and quark masses. For a Higgs mass of $m_H = 125~{\rm GeV}$ and an LHC center-of-mass energy of $13~{\rm TeV}$, our best prediction for the gluon fusion cross-section is \[ \sigma = 48.58\,{\rm pb} {}^{+2.22\, {\rm pb}\, (+4.56\%)}_{-3.27\, {\rm pb}\, (-6.72\%)} \mbox{ (theory)} \pm 1.56 \,{\rm pb}\, (3.20\%) \mbox{ (PDF+$\alpha_s$)} \]

==> table_sigmas_7Tev_HXSWG.tex <==
\begin{table}[h!]
\normalsize\setlength{\tabcolsep}{2pt}
\begin{center}
\begin{tabular}{ccccccccccc}
\toprule
\begin{tabular}{c} $m_H$ \\(GeV) \end{tabular} & 
\begin{tabular}{c} $\sigma(m_H/2)$\\(pb) \end{tabular}& 
\begin{tabular}{c} $\delta(PDF)$\\(pb) \end{tabular}& 
\begin{tabular}{c} $\delta(\alpha_s)$\\(pb) \end{tabular} &
\begin{tabular}{c} $\delta$(scale)\\(pb) \end{tabular} &
\begin{tabular}{c} $\delta$(trunc)\\(pb) \end{tabular} &
\begin{tabular}{c} $\delta$(pdfTH)\\(pb) \end{tabular} &
\begin{tabular}{c} $\delta$(EW)\\(pb) \end{tabular} & 
\begin{tabular}{c} $\delta$(tb) \\(pb) \end{tabular} & 
\begin{tabular}{c} $\delta(1/m_t)$\\(pb) \end{tabular}\\ \midrule
120 & 18.30 & $\pm$ ?  & $\pm$ ? & $\pm$ 0.05
&$\pm$? & $\pm$ ? & $\pm$ ? & $\pm$ ? & $\pm$ ? \\ \midrule
120.5 & 18.30 & $\pm$ ?  & $\pm$ ? & $\pm$ 0.20
&$\pm$? & $\pm$ ? & $\pm$ ? & $\pm$ ? & $\pm$ ? \\ \midrule
130 & 18.30 & $\pm$ ?  & $\pm$ ? & $\pm$ 2.81
&$\pm$? & $\pm$ ? & $\pm$ ? & $\pm$ ? & $\pm$ ? \\ \midrule
\end{tabular}
\end{center}
\caption{Gluon-fusion Higgs cross-section and breakdown of the error budget, in \%, relative
to the total cross-section (column 2)}
\label{tab:xs_relerr}
\end{table}
